IV-Bench: A Benchmark for Image-Grounded Video Perception and Reasoning in Multimodal LLMs

Existing evaluation frameworks for Multimodal Large Language Models (MLLMs) primarily focus on image reasoning or general video understanding tasks, largely overlooking the significant role of image context in video comprehension. To bridge this gap, we propose IV-Bench, the first comprehensive benchmark for evaluating Image-Grounded Video Perception and Reasoning. IV-Bench consists of 967 videos paired with 2,585 meticulously annotated image-text queries across 13 tasks (7 perception and 6 reasoning tasks) and 5 representative categories. Extensive evaluations of state-of-the-art open-source (e.g., InternVL2.5, Qwen2.5-VL) and closed-source (e.g., GPT-4o, Gemini2-Flash and Gemini2-Pro) MLLMs demonstrate that current models substantially underperform in image-grounded video Perception and Reasoning, merely achieving at most 28.9% accuracy. Further analysis reveals key factors influencing model performance on IV-Bench, including inference pattern, frame number, and resolution. Additionally, through a simple data synthesis approach, we demonstratethe challenges of IV- Bench extend beyond merely aligning the data format in the training proecss. These findings collectively provide valuable insights for future research. Our codes and data are released in https://github.com/multimodal-art-projection/IV-Bench.

==> sections/Acknowledgements.tex <==


\section{Acknowledgements}
Multimodal Art Projection (M-A-P) is an open-source AI research community.
The community members are working on research topics in a wide range of spectrum, including but not limited to pre-training paradigm of foundation models, large-scale data collection and processing, and the derived applciations on coding, reasoning and music generation.



==> sections/demos.tex <==
\section{IV Bench Demo}

During model inference, we construct multiple-choice questions and randomly shuffle the answer and distractors, with the position of the correct answer randomized. The default placement order is video, image, and text. For some models, we also experiment with placing the image after the video. Therefore, we have two different text prompts: one with the order of video, image, and text, and another with the image placed after the video. In the prompt, we explicitly specify the order of the video and image, the video length, and instruct the model to answer the question based on both the video and the image, providing only the options.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{pic/demos/attribute_change_AND_constrained_ocr.png}
    \caption{attribute change (left) and constrained ocr (right)}
    \label{fig:attribute_change_AND_constrained_ocr}
\end{figure}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{pic/demos/counting_AND_details_event.png}
    \caption{counting (left) and constrained details event (right)}
    \label{fig:counting_AND_details_event}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{pic/demos/instruction_manual_AND_keyframe_extraction.png}
    \caption{instruction manual (left) and keyframe extraction (right)}
    \label{fig:instruction_manual_AND_keyframe_extraction}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{pic/demos/space-time_computing_AND_temporal_reasoning.png}
    \caption{space-time computing (left) and temporal reasoning (right)}
    \label{fig:space-time_computing_AND_temporal_reasoning}
\end{figure}



==> sections/discussion.tex <==
\section{Discussion}

==> table/review_info/human_check.tex <==
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llp{12cm}}
    \toprule 
    \textbf{Category} & \textbf{Focus} & \textbf{Description} \\
    \midrule 
    \multirow{13}{*}{\raisebox{-10ex}{\raisebox{-1ex}{\includegraphics[width=0.5cm]{pic/review/question.png}} \quad \textbf{Question}}} & \multirow{1}{*}{Source Consistency} & Align question source with annotations. \\
    \cmidrule(lr){3-3} 
    \cmidrule(lr){2-3} 
    & \multirow{2}{*}{Condition Completeness} & Base answers solely on provided text. \\
    \cmidrule(lr){3-3} 
    & & Avoid needing additional conditions like charts or legal clauses. \\
    \cmidrule(lr){2-3} 
    & \multirow{3}{*}{Question Clarity} & Be clear and specific. \\
    \cmidrule(lr){3-3} 
    & & Have only one correct answer. \\
    \cmidrule(lr){3-3} 
    & & Avoid vague or open-ended questions. \\
    \cmidrule(lr){2-3} 
    & \multirow{3}{*}{Expression Accuracy} & Write in English. \\
    \cmidrule(lr){3-3} 
    & & Use precise terminology. \\
    \cmidrule(lr){3-3} 
    & & Accurately translate specialized terms. \\
    \cmidrule(lr){2-3} 
    & \multirow{2}{*}{Formula and Numerical Accuracy} & Write formulas in LaTeX. \\
    \cmidrule(lr){3-3} 
    & & Align key formulas and numerical details. \\
    \cmidrule(lr){2-3} 
    & \multirow{2}{*}{Global Perspective} & Frame from a global perspective. \\
    \cmidrule(lr){3-3} 
    & & Avoid regional bias. \\
    \midrule 
    \multirow{6}{*}{\raisebox{-5ex}{\raisebox{-1ex}{\includegraphics[width=0.5cm]{pic/review/options.png}} \quad \textbf{Options}}} & \multirow{1}{*}{Expression Accuracy} & Accurately translate proper nouns and terminology. \\
    \cmidrule(lr){3-3} 
    \cmidrule(lr){2-3} 
    & \multirow{2}{*}{Formula and Numerical Accuracy} & Ensure formula and numerical accuracy. \\
    \cmidrule(lr){3-3} 
    & & Correctly format in LaTeX. \\
    \cmidrule(lr){2-3} 
    & \multirow{3}{*}{Distractor Relevance} & Make incorrect options meaningful but not correct. \\
    \cmidrule(lr){3-3} 
    & & Distinguish from correct answers. \\
    \cmidrule(lr){3-3} 
    & & Match correct options in length and format. \\
    \midrule 
    \multirow{4}{*}{\raisebox{-3ex}{\raisebox{-1ex}{\includegraphics[width=0.5cm]{pic/review/answer.png}} \quad \textbf{Answer}}} & \multirow{2}{*}{Answer Correctness} & Ensure the answer is in the options. \\
    \cmidrule(lr){3-3} 
    & & Accurately answers the question. \\
    \cmidrule(lr){2-3} 
    & \multirow{2}{*}{Answer Uniqueness} & Ensure the answer is unique. \\
    \cmidrule(lr){3-3} 
    & & Avoid multiple valid answers due to vague wording or incorrect options. \\
    \midrule 
    \multirow{2}{*}{\raisebox{-1ex}{\raisebox{-1ex}{\includegraphics[width=0.5cm]{pic/review/speedometer.png}} \quad \textbf{Difficulty}}} & \multirow{1}{*}{Difficulty Matching} & Match difficulty to graduate-level. \\
    \cmidrule(lr){3-3} 
    \cmidrule(lr){2-3} 
    & \multirow{1}{*}{Difficulty Reasonableness} & Ensure difficulty is reasonable based on complexity and presented options. \\
    \midrule 
    \multirow{3}{*}{\raisebox{-2ex}{\raisebox{-1ex}{\includegraphics[width=0.5cm]{pic/review/book.png}} \quad \textbf{Discipline}}} & \multirow{1}{*}{Category Accuracy} & Categorize correctly with accurate primary and secondary subjects. \\
    \cmidrule(lr){2-3} 
    & \multirow{2}{*}{Category Validity} & Correctly fill category fields. \\
    \cmidrule(lr){3-3} 
    & & No missing or unnecessary fields. \\
    \bottomrule 
\end{tabular}
}
\caption{human check}
\end{table}


==> table/review_info/rule_check.tex <==
\begin{table}[ht]
\centering
\label{Tab: Rule_Check}
\resizebox{\textwidth}{!}{
\begin{tabular}{l p{16cm}}
    \toprule 
    \textbf{Category} & \textbf{Rules} \\
    \midrule
    \multirow{4}{*}{\raisebox{-3ex}{\raisebox{-1ex}{\includegraphics[width=0.5cm]{pic/review/text.png}} \quad \textbf{Text}}}
    & Replace full-width punctuation with half-width punctuation. \\
    \cmidrule(lr){2-2}
    & Remove unnecessary whitespace characters (e.g., spaces, newline characters, tab spaces). \\
    \cmidrule(lr){2-2}
    & Replace common escape characters. \\
    \cmidrule(lr){2-2}
     & Add missing escape characters. \\
    \midrule
    \multirow{8}{*}{\raisebox{-15ex}{\raisebox{-1ex}{\includegraphics[width=0.5cm]{pic/review/question.png}}\quad\textbf{Question}}} 
    & Not Empty or Placeholder. \\
    \cmidrule(lr){2-2}
    & Ensure the question field is in string format to avoid errors. \\
    \cmidrule(lr){2-2}
    & Text length \textgreater \, 5.  \\
    \cmidrule(lr){2-2}
    & Text Standardization. \\
    \cmidrule(lr){2-2}
    & Perplexity \textleq 100, calculated using the \textit{Qwen2.5-0.5B-Instruct} model. \\
    \cmidrule(lr){2-2}
    & No Semantic Duplicates: For a given question \(q_i\), the cosine similarity with each existing question \(q_j\) :  
    \[ \text{CosineSimilarity}(q_i, q_j) = \frac{\mathbf{e_i} \cdot \mathbf{e_j}}{\|\mathbf{e_i}\| \|\mathbf{e_j}\|}<0.90 \]  where \(\mathbf{e_i}\) and \(\mathbf{e_j}\) are embeddings generated by the model SentenceTransformer("all-MiniLM-L6-v2"), and \textit{Faiss} is used for efficient similarity search. \\
    \midrule
    \multirow{5}{*}{\raisebox{-8ex}{\raisebox{-1ex}{\includegraphics[width=0.5cm]{pic/review/options.png}}\quad\textbf{Options}}}    
    & 4 \(\leq\) Option count \(\leq\) 10. \\
    \cmidrule(lr){2-2}
    & No empty or meaningless options (e.g., no empty strings, no only whitespace characters, no common placeholders like 'none', 'null'). \\
    \cmidrule(lr){2-2}
    & No duplicate options. \\
    \cmidrule(lr){2-2}
    & Remove built-in option prefixes\\
    \cmidrule(lr){2-2}
    & Text Standardization for each option. \\
    \midrule
    \multirow{3}{*}{\raisebox{-3ex}{\raisebox{-1ex}{\includegraphics[width=0.5cm]{pic/review/answer.png}}\quad\textbf{Answer}}}   
    & Not Empty or Placeholder. \\
    \cmidrule(lr){2-2}
    & Within options list. \\
    \cmidrule(lr){2-2}
    & Text Standardization. \\
    \midrule
    \raisebox{-0.8ex}{\includegraphics[width=0.5cm]{pic/review/speedometer.png}}\quad\textbf{Difficulty}    
    & Ensure difficulty exists. \\
    \midrule
    \raisebox{-0.8ex}{\includegraphics[width=0.5cm]{pic/review/book.png}}\quad\textbf{Discipline}  
    & Ensure discipline, field, and subfield exist. \\
    \bottomrule
\end{tabular}
}
\caption{Rule-Based Pre-Check}
\end{table}

